Wispy to Voluminous: Prior-free Multi-view Capture of Strand-level Facial Hair

Facial hair is a defining trait of personal identity, yet remains a critical bottleneck for digital avatars. Recent volumetric methods achieve photorealism but bake hair into the underlying face geometry, preventing editability and failing to resolve sparse, strand-like structures. Meanwhile, scalp-hair reconstruction methods target dense hair volumes and do not transfer to the sparse, spatially-varying nature of facial hair. We present a pipeline that automatically reconstructs facial hair -- beard, mustache, lashes, and brows -- from multi-view images, converting an unstructured 3D Gaussian representation into an explicit curve-based strand representation. We resolve geometric ambiguities in four stages: (i) optimizing 3D Gaussians constrained by tracked head geometry to enforce early ray termination and suppress sub-surface noise; (ii) tracing continuous strands robust to frequent crossings and extreme curvature; (iii) grounding strands to the surface and resolving root-tip ambiguity via a physically-motivated prior; and (iv) refining the reconstruction through opacity-driven density control under photometric optimization. To our knowledge, this is the first method to reconstruct high-fidelity facial hair strands from a 3D Gaussian representation. The recovered strands faithfully preserve the orientation and sparsity patterns characteristic of facial hair, and yield assets immediately suitable for downstream production tasks, including facial animation and physical simulation, geometric grooming and transfer, appearance editing, and physics-based rendering.

==> Tables/1_cg_test_baseline_comp.tex <==
\begin{table*}[h]
\centering
\caption{Comparison to state-of-the-art video animation methods on our self-collected hair motion test-set.}\vspace{-10pt}
\label{tab:cg_test_set}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc|ccccc|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Hair}} & \multicolumn{5}{c|}{\textbf{Full Body}} & \multirow{2}{*}{\textbf{Avg Infer Time(s)$\downarrow$}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
& \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{cd-FVD$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{cd-FVD$\downarrow$} & \\
\midrule
LTX-Video-0.9.8-13B~\citep{HaCohen2024LTXVideo} & 0.9642 & 30.3565 & 0.0468 & 156.8218 & 827.5890 & 0.7885 & 19.9854 & 0.2751 & 113.9513 & 866.8544 & \textbf{56} \\
Wan-2.2-14B~\citep{wan2025} & 0.9153 & 24.8174 & 0.1326 & 172.6361 & 802.6791 & 0.5535 & 12.7273 & 0.6345 & 89.8836 & 868.1351 & 476 \\
LTX-Video-ICLora~\citep{HaCohen2024LTXVideo}& {0.9700} & 30.6511 & 0.0365 & 108.1872 & 652.3275 & 0.8665 & 24.1449 & 0.1446 & 45.4541 & {423.4040} & \underline{58} \\

UniAnimate-DiT~\citep{wang2025unianimate} & \underline{0.9761} & \underline{35.4174} & {0.0304} & 66.1997 & 678.9257 & \underline{0.8724} & \underline{25.6764} & \underline{0.1407} & \underline{45.0817} & \underline{448.8855} & 870 \\

Wan-2.2-Animate-14B~\citep{wan2025} & 0.9758 & {35.3174} & \underline{0.0299} & \underline{59.6534} & \underline{587.4605} & 0.8400 & 25.2877 & 0.1803 & 49.4041 & {461.6013} & 312 \\

\ourmodel & \textbf{0.9794} & \textbf{37.6347} & \textbf{0.0233} & \textbf{50.5938} & \textbf{434.1582} & \textbf{0.8948} & \textbf{27.7903} & \textbf{0.1127} & \textbf{43.2786} & \textbf{407.1929} & {62} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Tables/2_cg_test_ablation.tex <==
\begin{table*}[h]
\centering
\caption{Ablation Analysis. \textbf{DiT+Pose Encoder} denotes the DiT backbone is trained with Pose Encoder only without \domain and \pose. \textbf{DiT+Pose-IC-LoRA} denotes the DiT backbone is trained with In-Context-Lora, the same as LTX-Video-ICLora~\citep{HaCohen2024LTXVideo}, without \domain and \pose. \textbf{w/o \domain} denotes the \domain module is removed from the \ourmodel pipeline.} 
\vspace{-10pt}
\label{tab:cg_test_ablation}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Hair}} & \multicolumn{5}{c}{\textbf{Full Body}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
& \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{cd-FVD$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{cd-FVD$\downarrow$} \\
\midrule
DiT+Pose Encoder & 0.9158 & 27.4486 & 0.1214 & 94.0048 & 654.8677 & 0.5623 & 12.9256 & 0.6481 & 91.1008 & 431.4920 \\

DiT+Pose-IC-LoRA& \underline{0.9700} & 30.6511 & 0.0365 & 108.1872 & 652.3275 & 0.8665 & 24.1449 & 0.1446 & 45.4541 & {423.4040} \\
w/o \domain & 0.9693 & \underline{36.7183} & \underline{0.0236} & \textbf{49.0808} &  \underline{447.7628}& \underline{0.8828} & \underline{26.5544} & \underline{0.1184} & \textbf{38.4230} & \underline{416.9271} \\
\ourmodel & \textbf{0.9794} & \textbf{37.6347} & \textbf{0.0233} & \underline{50.5938} & \textbf{434.1582} & \textbf{0.8948} & \textbf{27.7903} & \textbf{0.1127} & \underline{43.2786} & \textbf{407.1929} \\


\bottomrule
\end{tabular}
}

\end{table*}

==> Tables/3_user_study.tex <==
\begin{table}[htp]
\centering
\caption{The user study with 30 participants. We collect the number of votes for eight video subjects from test set by six methods and report the average percentage. (Full table presented in the supplement). Our \ourmodel generates the most realistic human videos with hair motions.
}
\label{tab:user_study}
\scalebox{1.0}
{\begin{tabular}{lcccccccccccc}
\toprule
Method  & {\textbf{Average}}\\
\midrule
LTX-Video-0.9.8-13B~\citep{HaCohen2024LTXVideo} & 6.9\%\\

Wan-2.2-14B~\citep{wan2025} & 8.2\%\\
LTX-Video-ICLora~\citep{HaCohen2024LTXVideo} & 9.0\%\\
UniAnimate-DiT~\citep{wang2025unianimate} & 9.5\%\\
Wan-2.2-Animate-14B~\citep{wan2025} & \underline{16.4\%}\\
\ourmodel & \textbf{49.9\%}\\
\bottomrule
\end{tabular}}
\end{table}



==> Tables/4_ns_test_set.tex <==
\begin{table*}[h]
\centering
\caption{Comparison to state-of-the-art video animation methods on NeRSemble~\citep{kirschstein2023nersemble} test-set.}\vspace{-10pt}
\label{tab:ns_test_set}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Hair}} & \multicolumn{5}{c}{\textbf{Portrait}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
& \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{cd-FVD$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{cd-FVD$\downarrow$} \\
\midrule
LTX-Video-0.9.8-13B~\citep{HaCohen2024LTXVideo} & 0.9131 & 23.40 & 0.1020 & 120.74 & 891.18 & 0.6871 & 17.83 & 0.3878 & 73.50 & 703.35 \\
Wan-2.2-14B~\citep{wan2025} & 0.9150 & 21.65 & 0.1051 & 113.11 & 652.18 & 0.6865 & 17.28 & 0.3830 & 51.43 & 503.07 \\
LTX-Video-ICLora~\citep{HaCohen2024LTXVideo} & 0.9397 & 24.95 & 0.0710 & 44.11& 384.41 & 0.7635 &20.99 &0.2683 &28.42 & \underline{277.77} \\
UniAnimate-DiT~\citep{wang2025unianimate} & 0.9350 & 25.33 & 0.0810 & 66.29 & 477.13 & 0.7545 & 20.32 & 0.3059 & 52.44 & 379.12 \\
Wan-2.2-Animate-14B~\citep{wan2025} & \underline{0.9544} & \underline{28.75} & \underline{0.0599} & \underline{20.48} & \underline{328.67} & \underline{0.8011} & \underline{23.62} & \underline{0.2030} & \underline{24.32} & {314.65} \\
\ourmodel & \textbf{0.9670} & \textbf{34.34} & \textbf{0.0477} & \textbf{17.79} & \textbf{286.25} & \textbf{0.8291} & \textbf{26.47} & \textbf{0.1763} & \textbf{19.43} & \textbf{212.61} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Tables/5_user_study_full.tex <==
\begin{table*}[]
\centering
\caption{The user study with 30 participants. We collect the number of votes for eight video subjects from test set by six methods and report the percentage. Our \ourmodel generates the most realistic human videos with hair motions.
}
\label{tab:user_study_full}
\scalebox{0.7}
{\begin{tabular}{lcccccccccccc}
\toprule
Method  & {\textbf{Subject1}} & {\textbf{Subject2}}& {\textbf{Subject3}}& {\textbf{Subject4}}&{\textbf{Subject5}} & {\textbf{Subject6}} & {\textbf{Subject7}}& {\textbf{Subject8}}& {\textbf{Average}}\\
\midrule
LTX-Video-0.9.8-13B~\citep{HaCohen2024LTXVideo} & 0.0\% & 6.9\% & 10.3\% & 10.3\% & 6.9\% & {10.3\%} & 6.9\% & 3.4\% & 6.9\%\\
Wan-2.2-14B~\citep{wan2025} & 10.3\% & 3.4\% & 10.3\% & 10.3\% & 3.4\% & 6.9\% & 6.9\% & 13.8\% & 8.2\%\\
LTX-Video-ICLora~\citep{HaCohen2024LTXVideo} & \underline{20.7\%} & 6.9\% & 6.9\% & 10.3\% & \underline{10.3\%} & 6.9\% & 6.9\% & 3.4\% & 9.0\%\\
UniAnimate-DiT~\citep{wang2025unianimate} & 10.3\% & 10.3\% & 10.3\% & 10.3\% & 6.9\% & 6.9\% & \underline{17.2\%} & 3.4\% & 9.5\%\\
Wan-2.2-Animate-14B~\citep{wan2025} & 10.3\% & \underline{24.1\%} & \underline{17.2\%} & \underline{24.1\%} & 6.9\% & \underline{13.8\%} & 6.9\% & \underline{27.6\%} & \underline{16.4\%}\\
\ourmodel & \textbf{48.3\%} & \textbf{48.3\%} & \textbf{41.4\%} & \textbf{34.5\%} & \textbf{65.5\%} & \textbf{55.2\%} & \textbf{55.2\%} & \textbf{48.3\%} & \textbf{49.9\%}\\
\bottomrule
\end{tabular}}
\end{table*}

==> Tables/6_user_study_oculus.tex <==

\begin{table}[]
\centering
\caption{A larger-scale user study with 45 participants on 20 videos. We collect the number of votes for these 20 video subjects from test set by six methods and report the average percentage. Our \ourmodel generates the most realistic human videos with hair motions.
}
\label{tab:user_study_oculus}
\scalebox{1.0}
{\begin{tabular}{lcccccccccccc}
\toprule
Method  & {\textbf{Average}}\\
\midrule
LTX-Video-0.9.8-13B~\citep{HaCohen2024LTXVideo} & 1.83\%\\

Wan-2.2-14B~\citep{wan2025} & 3.78\%\\
LTX-Video-ICLora~\citep{HaCohen2024LTXVideo} & 4.02\%\\
UniAnimate-DiT~\citep{wang2025unianimate} & 6.95\%\\
Wan-2.2-Animate-14B~\citep{wan2025} & \underline{15.24\%}\\
\ourmodel & \textbf{68.17\%}\\
\bottomrule
\end{tabular}}
\end{table}
